A Survey of Generative AI for Intelligent Transportation Systems: Road Transportation Perspective

Intelligent transportation systems are vital for modern traffic management and optimization, greatly improving traffic efficiency and safety. With the rapid development of generative artificial intelligence (Generative AI) technologies in areas like image generation and natural language processing, generative AI has also played a crucial role in addressing key issues in intelligent transportation systems (ITS), such as data sparsity, difficulty in observing abnormal scenarios, and in modeling data uncertainty. In this review, we systematically investigate the relevant literature on generative AI techniques in addressing key issues in different types of tasks in ITS tailored specifically for road transportation. First, we introduce the principles of different generative AI techniques. Then, we classify tasks in ITS into four types: traffic perception, traffic prediction, traffic simulation, and traffic decision-making. We systematically illustrate how generative AI techniques addresses key issues in these four different types of tasks. Finally, we summarize the challenges faced in applying generative AI to intelligent transportation systems, and discuss future research directions based on different application scenarios.

==> Tabels/sec6.1.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[ht]
\begin{center}
\begin{tabular}{c|l|l|l}
\hline
\textbf{Categories}                   & \textbf{Method}           & \textbf{Papers}  & \textbf{Application}  \\ \hline
\hline
\multirow{2}{*}{Domain decomposition} & knowledge-driven          & cite{}           &                       \\ \cline{2-4} 
                                      & data-driven               & cite{}           &                       \\ \hline
\multirow{2}{*}{Multigrid method}     & theory-guided             & cite{}           &                       \\ \cline{2-4}
                                      & technique-introduced      & cite{}           &                       \\ \hline
\end{tabular}
\end{center}
\caption{TYPE A}\label{Tab:type-a}
\end{table*}

==> Tabels/sec6.2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[ht]
\begin{center}
\begin{tabular}{c|l|l|l}
\hline
\textbf{Categories}                                    & \textbf{Method}           & \textbf{Papers}   & \textbf{Application}  \\ \hline
\hline
\multirow{2}{*}{Data-driven}                           & FEA                       & \cite{}           &                       \\ \cline{2-4} 
                                                       & REV                       & \cite{}           &                       \\ \hline
\multirow{2}{*}{Knowledge-driven}                      & NN surrogated DFT         & \cite{}           &                       \\ \cline{2-4}
                                                       & NN surrogated FEA         & \cite{}           &                       \\ \hline
\multirow{2}{*}{Knowledge and data jointly driven}     & NN enhanced FEA           & \cite{}           &                       \\ \cline{2-4}
                                                       & NN enhanced REV           & \cite{}           &                       \\ \hline
\end{tabular}
\end{center}
\caption{TYPE B}\label{Tab:typeb}
\end{table*}

==> Tabels/sec6.3.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[ht]
\begin{center}
\begin{tabular}{c|l|l|l}
\hline
\textbf{Categories}                                    & \textbf{Method}           & \textbf{Papers}   & \textbf{Application}  \\ \hline
\hline
\multirow{2}{*}{Knowledge-driven}                      & Boundary-constraint       & \cite{}           &                       \\ \cline{2-4} 
                                                       & Overlap interaction       & \cite{}           &                       \\ \hline
\multirow{2}{*}{Data-driven}                           & Sampling-based            & \cite{}           &                       \\ \cline{2-4}
                                                       & Fitting-based             & \cite{}           &                       \\ \hline
\end{tabular}
\end{center}
\caption{TYPE C}\label{Tab:typec}
\end{table*}

==> Tabels/sec6.4.tex <==
\begin{table}[]
\centering
\setlength{\leftmargini}{0.4cm}
\begin{tabular}{m{4cm} | m{5cm} | m{4cm} }
\hline
\textbf{Category} & \textbf{Method} & \textbf{Examples} \\ \hline\hline
Scale with linear properties & Dynamic mode decomposition~\cite{schmid2010dynamic,kutz2016dynamic,proctor2016dynamic,tu2013dynamic} & ~\cite{schmid2011applications,hemati2014dynamic,habibi2020data} \\ \hline
\multirow{4}{*}{\makecell[c]{Scale with preserved \\ relevant information}}
& Causal emergence & \cite{griebenow2019finding,hoel2013quantifying} \\ \cline{2-3} 
 & Coarse-scale partial differential equations & \cite{bar2019learning,lee2020coarse} \\ \cline{2-3} 
 & Slow variables & \cite{perez2013identification,singer2009detecting,noe2013variational,wehmeyer2018time,bramburger2020sparse}\\ \cline{2-3} 
 & Governing equations  & \cite{champion2019data, brunton2016discovering, huang2018mesoscience, chen2022automated} \\ \cline{2-3}
 & Renormalization group &  \cite{koch2018mutual,li2018neural,di2022deep} \\ \hline
\end{tabular}%
\caption{Multi-scale modeling and simulation methods to achieve {\em Objective D}}
\end{table}


==> Tabels/sec6.5.tex <==
\begin{table}[]
\centering
\setlength{\leftmargini}{0.4cm}
\begin{tabular}{m{4cm} | m{5cm} | m{4cm} }
\hline
\textbf{Category} & \textbf{Method} & \textbf{Examples} \\ \hline\hline
\multirow{3}{*}{Knowledge-driven} & Wavelet-based methods &  \cite{mallat1989theory,beylkin1998multiresolution,gilbert1998comparison,mehraeen2006wavelet}\\ \cline{2-3}
& Multiscale homogenization & \cite{chen2006generalized,yu2002multiscale,li2008generalized}\\ \cline{2-3}
& Stochastic methods & \cite{chen2006generalized,yu2002multiscale,li2008generalized}\\ \hline

\multirow{3}{*}{\makecell[c]{Data-driven}}
& Autoencoders & \cite{vlachas2021accelerated,vlachas2022multiscale,lee2020model,fukami2020convolutional,hernandez2018variational} \\ \cline{2-3} 
 & Neural ODEs & \cite{chen2018neural,maulik2020time,maulik2021reduced}\\ \cline{2-3}
 & Sampling strategies & \cite{champion2019discovery,bhatia2021machine,gong2021advanced,dupuis2012importance,manohar2019optimized}\\ \hline
\end{tabular}%
\caption{Multi-scale modeling and simulation methods to achieve {\em Objective E}}
\end{table}

==> Tabels/sec6_tbl.tex <==
\begin{table}[]
\centering
\setlength{\leftmargini}{0.4cm}
\begin{tabular}{m{2cm} | m{2cm} | m{5cm} | m{6cm} }
\hline
\textbf{Category1} & \textbf{Category2} & \textbf{xxx} & \textbf{Examples and applications} \\ \hline\hline
\multirow{3}{*}{\makecell[c]{Clear\\scales}}   & Type A & 
\begin{itemize}
    \item Domain decomposition~\cite{brooks2009charmm,fish2021mesoscopic,mosser2017reconstruction,yang2018microstructural,wang2019meta,liu2016self,wang2019coarse,mikolov2010recurrent,wu2020recurrent}
    \item Multigrid~\cite{miehe2007multiscale,gravemeier2010algebraic,yushu2020image,dai2019excmg}
\end{itemize}
&  \\ 
                                & Type B & 
\begin{itemize}
    \item Knowledge-driven~\cite{sridhar2016homogenization,ozdemir2008computational,yuan2009multiple}
    \item Data-driven~\cite{allam2018application,le2015computational,xie2018crystal}
    \item Data and knowledge jointly driven~\cite{karniadakis2021physics,hambli2011multiscale,oishi2017computational}
\end{itemize}
&  \\ 
                                & Type C & 
\begin{itemize}
    \item Knowledge-driven~\cite{tao2010nonintrusive,chakraborty2018hyperdynamics,guo2016multi}
    \item Data-driven~\cite{ingolfsson2022machine,bhatia2021machine,han2017deep}
\end{itemize}
&  \\ \hline
\multirow{2}{*}{\makecell[c]{Unclear\\scales}} & Type D & 
\begin{itemize}
    \item Discovering unknown scales~\cite{hoel2013quantifying,hoel2016can,champion2019discovery}(slow scales, linear scale, coarse scale)
    \item Discovering governing equations~\cite{brunton2016discovering,champion2019data,maulik2021reduced}
    %\item Discovering slow variables~\cite{bramburger2020sparse,wehmeyer2018time,noe2013variational,singer2009detecting,perez2013identification}
\end{itemize}
&   \\ 
& Type E & 
\begin{itemize}
    \item Knowledge-driven
    \item Data-driven~\cite{}
\end{itemize}
                                &  \\ \hline
\end{tabular}%
\end{table}

